quantum Case-Based Reasoning (qCBR)

Case-Based Reasoning (CBR) is an artificial intelligence approach to problem-solving with a good record of success. This article proposes using Quantum Computing to improve some of the key processes of CBR, such that a Quantum Case-Based Reasoning (qCBR) paradigm can be defined. The focus is set on designing and implementing a qCBR based on the variational principle that improves its classical counterpart in terms of average accuracy, scalability and tolerance to overlapping. A comparative study of the proposed qCBR with a classic CBR is performed for the case of the Social Workers' Problem as a sample of a combinatorial optimization problem with overlapping. The algorithm's quantum feasibility is modelled with docplex and tested on IBMQ computers, and experimented on the Qibo framework.

==> images/back.tex <==
\begin{table}[t!]
    \centering
    \begin{tabular}{c|c|c}
      \hline
        Initial\_point  &  Schedule  &  Solution Class \\
         \hline
         &   &   &
          \hline
    \end{tabular}
    \caption{(a) qCBR's Memory structure - Solution class}
    \label{tab:(a)sol_class}
    \begin{tabular}{c|c}
      \hline
        solution class   &   Schedule \\
         \hline
         &   &   
          \hline
    \end{tabular}
    \caption{(b) qCBR's Memory structure - Training data}
    \label{tab:(b)train_data}
    \begin{tabular}{c|c}
      \hline
        solution class   &   Schedule \\
        \hline
        &   &   
        \hline
        &   &
        \hline
        &   & 
        \hline
        Cross-validation - (Leave One Out) & -- \\
        \hline
        &   &
        \hline
        &   &   
        \hline
        &   &   
        \hline
    \end{tabular}
    \caption{(c) qCBR's Memory structure. The use the cross-validation technique helps to improve the quality of the classifier training\cite{Mic}. - Test data}
    \label{tab:(c)test_data}
\end{table}


\begin{table}[t!]
    \centering
    \begin{tabular}{c|c|c|c}
        solution class &  Initial\_point\_{1}  & ... &  Initial\_point\_{N} \\
         \hline
        A  &  ...   & ...   & ...  \\
         \hline
    \end{tabular}
    \caption{Memory structure used for the Training System. A label identifies each class. And in this case, A is one of the labels. For more detail, refer to the code \cite{Ade21}.}
    \label{tab:mem_struture}
\end{table}
